Algorithm-hardware co-design for Energy-Efficient A/D conversion in ReRAM-based accelerators

Deep neural networks are widely deployed in many fields. Due to the in-situ computation (known as processing in memory) capacity of the Resistive Random Access Memory (ReRAM) crossbar, ReRAM-based accelerator shows potential in accelerating DNN with low power and high performance. However, despite power advantage, such kind of accelerators suffer from the high power consumption of peripheral circuits, especially Analog-to-Digital Converter (ADC), which account for over 60 percent of total power consumption. This problem hinders the ReRAM-based accelerator to achieve higher efficiency. Some redundant Analog-to-Digital conversion operations have no contribution to maintaining inference accuracy, and such operations can be eliminated by modifying the ADC searching logic. Based on such observations, we propose an algorithm-hardware co-design method and explore the co-design approach in both hardware design and quantization algorithms. Firstly, we focus on the distribution output along the crossbar's bit-lines and identify the fine-grained redundant ADC sampling bits. % of weight and To further compress ADC bits, we propose a hardware-friendly quantization method and coding scheme, in which different quantization strategy was applied to the partial results in different intervals. To support the two features above, we propose a lightweight architectural design based on SAR-ADC\@. It's worth mentioning that our method is not only more energy efficient but also retains the flexibility of the algorithm. Experiments demonstrate that our method can reduce about $1.6 \sim 2.3 \times$ ADC power reduction.

==> tex/2_background_pool.tex <==
\section{Background and Motivation}\label{background}

% There are various ReRAM-based accelerator architectures~\cite{shafiee2016isaac,chi2016prime,zhu2018mixed}. In this section, we first introduce how the ReRAM-based accelerator works. Then we introduce how ADC quantizes the output current of the crossbar. 
\subsection{Analog PIM basic}

% The basic analog PIM macro consists of a ReRAM crossbar and peripheral circuits. 
% A ReRAM crossbar has $\#Row \times \#Col$ ReRAM cells, and the peripheral circuits include ADC, DAC, multiplexer, decoder, etc. 
% As shown in Fig.~\ref{im_substract}, to enable the analog computation, the weights are stored as the conductance of the ReRAM cells ($\mathbf{G}$);

\paragraph*{\textbf{PIM macro}}
The basic analog PIM macro consists of a ReRAM crossbar array and peripheral circuits such as the peripheral circuits include ADC, DAC, multiplexer, decoder, etc., as shown in Fig.~\ref{im_substract}. 
When performing the analog computation, the weights are stored as the conductance of the ReRAM cells ($\mathbf{G}$);
and input vectors ($\bm{x}$) are converted to voltage vectors ($\mathbf{V}$) at word lines (WLs) by DAC\@. 
Currents through each cell, representing the scalar multiplication results, accumulate along the BLs, i.e., $\mathbf{I}_i=\sum_j \mathbf{G}_{i,j}\mathbf{V}_j$. 
ADC plays an important role that converting currents at each BL to digital outputs. 
\begin{figure}[tbhp]
    \centering
    \includegraphics[width=0.95\linewidth]{ims/pdf/2_subtract.pdf}
    \caption{Demonstration of computation of matrix-vector multiplication with two ReRAM crossbars. 
The left is the separation of the weight into a positive part and a negative part. 
The right is the computation on hardware.}%
    \label{im_substract}
   % \Description{}
    %\vspace{-0.4cm}
\end{figure}
% Because the ReRAM crossbar can hold only positive weights, a weight matrix $\mathbf{W}$ is represented by mapped into a crossbar pair. 
Because the ReRAM crossbar can hold only positive weights, 
a weight matrix $\mathbf{W}$ is represented by mapped into a crossbar pair. 
As shown in Figure~\ref{im_substract}, 
$\mathbf{W}$ is separated into a positive part ($\mathbf{W^{+}}$) and a negative part ($\mathbf{W^{-}}$). 
The output currents from the two parts are subtracted in the analog domain, 
which is formulated as Eq.~\ref{computation_negative}. 
\begin{equation}
\label{computation_negative}
    \mathbf{I}_i=\sum_j \mathbf{G}_{i,j}^+\mathbf{V}_j-\sum_j \mathbf{G}_{i,j}^- \mathbf{V}_j
\end{equation}
% \subsection{Map Neural Networks to Accelerator}

\paragraph*{\textbf{Map Neural Networks to Accelerator}} 
The dense MVMs in DNNs such as fully-connected layers (FC) and convolutional layers (Conv2d) are mapped to the PIM macros. 
As shown in Fig.~\ref{fig::base_mapping}, 
a convolutional kernel (with $k \times k$ kernels, $C_i$ input channels) is transformed to MVM in different sliding windows~\cite{song2017pipelayer}. 
Fully connected layers can be seen as convolutional layers with $1\time1$ kernel size. 
When not fitting into a crossbar pair, a layer is split and mapped to multiple crossbars. 
As ReRAM cells can only store low bit values (up to 2 bits of recent fabrication technique~\cite{IRDS21MM}), 
weight values are represented by bitwise slices mapped to different BLs. 
% Although the state-of-art fabrication technique supports 2-bit cells~\cite {IRDS21MM}, 
% the no linearity of the conductance has not been well-solved, we use single-bit cells. 
% Different bitwise slices of weight are mapped to different BLs of the crossbar. 
Then, a shift-and-add and accumulator are needed to merge the partial sums to the final MVM result.
\begin{figure}[tbhp]
    \centering
    \includegraphics[width=0.99\linewidth]{ims/pdf/basic_mapping.drawio.pdf}
    \caption{Mapping convolutional layers. $K_w, K_i$ are the bit-width of the weight and input activation respectively.}%
    \label{fig::base_mapping}
   % \Description{}
    %\vspace{-0.4cm}
\end{figure}


The \textbf{intermediate activations (IA)} are merged to obtain the \textbf{merged activation (MA)}. 
Note that the ADC introduces extra quantization errors, which accumulate during the merging progress. 
Other types of layers execute either on functional units or coprocessors. 

\subsection{Quantization}
Quantization is one of the most effective techniques to compress neural networks. 
The uniform quantization projects a real number $x$ to a $k$-bit integer value $x_q$ with the scaling factor $\Delta_x$:
\begin{equation}
    x\approx\Delta_x x_q=Q_k(x,\Delta)=\Delta_x \text{clamp}(\text{round}(\frac{x}{\Delta_x}),0,2^{k}-1),
    \label{sym_quant}
\end{equation}
where $\text{round}$ projects a value to an integer and $\text{clamp}$ limits the output to the range that a $k$-bit integer can represent. 
There are two types of quantization methods, Quantization-Aware Training (QAT)~\cite{PACT_arxiv2018} and post-training quantization (PTQ)~\cite{PTQ_4bit_rapid_deployment_nips2019}. 
% QAT methods optimize both the weights and the quantization parameters to minimize task loss. 
% Though QAT may achieve aggressive quantization, it consumes extra training time and requires access to the training dataset. 
% Such two conditions are often unrealistic for the users and the hardware designers. 
Although QAT may achieve aggressive quantization, it consumes extra training time and requires access to the training dataset.
% In contrast, PTQ methods~\cite{Low_bit_quant_iccvw2019, EasyQuant_arxiv2020} require no network parameter and do not require a labeled dataset. 
In contrast, PTQ methods~\cite{Low_bit_quant_iccvw2019} require no extra training process.
In this paper, we focus on the PTQ\@. 

\subsection{ADC Preliminaries}%
\label{ADC_preliminaries}
% ADC 很重要
% ADC 对于性能的影响, performance, accuracy, area, power
% 相关因素：
% arch（sharing，arithmetical），algorithm，
% conversion, ADC cycle
% Basic
ADC is a critical component in an analog PIM macro that affects the overall inference accuracy.
Lossless conversion requires ADC with a resolution no less than $R_{ADC, ideal}$, i.e.,
\begin{align}
    % &R_{DAC, ideal} &=& \log_2(\lceil S\rceil_2) + R_{DA} + R_{cell} + \delta,\\
    &R_{DAC, ideal} &=& \log_2(S) + R_{DA} + R_{cell} + \delta,\\
    &\delta &=& 0\; \text{if } R_{DA}\ge 1\text{ and }R_{cell} \ge 1\text{ else }-1, \notag
\end{align} 
where $R_{cell}, R_{DA}, S$ are the number of bits a cell represents, the resolution of DAC, and the size of the crossbar, respectively. 
% Such resolution can cover any weight and input distribution and ensure no quantization error is introduced. 
% Two issues should be considered when using ADCs, overhead, and quantization error. 
% First, Since the power and area of ADCs increase exponentially with the resolution, % todo: \az{~\cite{}}, 
% using high-resolution ADCs is not competitive in terms of power and area. 
% Consequently, ADC with lower resolution ($\leq 8$) and 1-bit DAC is preferred in taped out chips~\cite{liu202033, yao2020fully, shafiee2016isaac, zhu2018mixed}. 
% Second, ADC functions as a quantizer and introduces extra quantization error to intermediate partial MVM results. 
% This behavior was not the designer's intent and needed to be specifically considered in the DNN quantization algorithm design. 
The overall ADC energy is formulated as:
\begin{align}
    E_{ADC, total, dyn} =&\text{len (input)} 
    \times \text{size}_{w} \label{eq:N_MACs}  \\
    \times &\frac{K_w}{R_{cell}} \times \frac{K_i}{R_{DA}} \label{eq:N_Convs} \\
    \times &E_{convert},
\end{align}
% The overhead of ADC is highly correlated with its resolution ($R_{ADC}$).
As the power of ADC scales exponentially with ADC resolution $R_{ADC}$ high-resolution ADCs are not competitive in terms of power and area. 
% Although some ADC architecture shows better energy efficiency
% DAC Energy: Is a strong function of the switching scheme
% SAR ADCs compare favorably up to moderate SNR of 60 dB. 
% In this range, SAR converters strongly benefit from 
% small feature sizes (enabling small unit capacitances) 
% and their relatively low circuit complexity
% ADC Power:
% 1. Conversion rate:
% FOM “corner” around 100…300MHz
% beyond this point,
% energy per conversion-step begins to increase linearly with frequency
% power scales with the square of frequency
% 2. Resolution:
% x2, x4, x8 per adding a bit
% Lower bound: thermal knee, improves with technology scaling, moving to lower SNDR
To overcome this challenge, 
solutions proposed by recent works can be categorized into three orthogonal levels: 
circuit, architecture, mapping, and algorithm.
\begin{itemize}[leftmargin=*]
    \item At the algorithm level,
          low-bit quantization~\cite{qu2021asbp, zhu2019configurable, sun2020energy} is widely used to reduce the bit-width of the weight and input activation ($K_w, K_i$, Eq.~\ref{eq:N_Convs});
          and pruning techniques~\cite{ma2020tiny, Shin2022Effective, qu2021asbp} are used to reduce
          required MVMs per inference (Eq.~\ref{eq:N_MACs}).
    \item At the mapping stage,
          weight encoding is introduced to obtain smaller conductance values ($K_w$)~\cite{Andrulis2023RAELLA, shafiee2016isaac};
          weight slicing and input slicing is explored in {RAELLA}~\cite{Andrulis2023RAELLA}
          to trade off ADC resolution (i.e., $E_{convert}$) and the number of A/D conversions per MVM (Eq.~\ref{eq:N_Convs}).
          % crossbar-aware pruning~\cite{Shin2022Effective, qu2021asbp} is proposed to 
          % save crossbar arrays reducing the number of MAC operations/DNN layers.
    \item At the architecture level~\cite{shafiee2016isaac, liu202033, yao2020fully},
          1-bit DAC and 1-bit ReRAM cells ($R_{DA}, R_{cell} = 1$) are widely adopted,
          and $R_{DAC, ideal} = \log_2(S) + 1$.
          % and the input value is represented by 2's complement and sent to DAC as bit serials ($R_{DA}, R_{cell} = 1$),
          Multi-bit input fed to DAC as bit series, aggregated by shift-and-add operations.
          % For area, ADC is shared among all the BLs in a time division manner, 
          % and shift-and-add operations accumulate over the dimensions of BLs, crossbars, and input cycles (Fig.~\ref{fig::base_mapping}). 
          % Note that, at the sign bit cycle, the S+A operation is replaced by shift-and-subtract operations. 
    \item At the circuit level,
          ADCs are customized with a non-uniform quantization scheme~\cite{sun2020energy};
          or discard, with all the operations conducted in the analog domain.
\end{itemize}

\subsection{A/D operations and coding scheme}
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{ims/pdf/sar_base_2type.drawio.pdf}
    \caption{Conventional SAR ADC with (a) uniform and (b) non-uniform grid}%
    \label{fig::sar_adc}
\end{figure}
SAR logic performs a binary search 
to compare the input signal with a series of reference voltages generated by a digital-to-analog converter (DAC). 
Each comparison determines one bit of the output\footnote[1]{To distinguish from the ``cycle'' of the system clock, 
we use ``ADC cycle'' to refer to the time of ADC to generate one bit.\label{fn:adc}}, 
starting from the most significant bit (MSB) to the least significant bit (LSB).
The closest output level is used as the approximation of the sampled voltage.
$N$ bits are generated in $N$ ADC cycles, 
and \textit{the output code is the concatenation of the results of each search step}\footnote[2]{We refer to each step of generating 1-bit as one \textbf{A/D operation}, 
and the full progress as the \textbf{A/D conversion}}.

As shown in Fig.~\ref{fig::sar_adc}, the horizontal dash grid represents 
reference voltages generated by a DAC ($V_{DAC}$)\@, 
vertical dash grid represents the time steps, 
points ($\otimes$) represent the sampled values to be sensed out, 
arrows consist of searching traces. 
A K-bit SAR-ADC performs a Binary Search (BS) on the grid 
by comparing with K reference voltages $V_{ref, idx(k)}$, 
% $\frac{1}{2}V_{ref}$, $(\frac{D_{K-1}}{2}+\frac{1}{4})V_{ref}$, …, $(\frac{D_{K-1}}{2}+\frac{D_{K-2}}{4} + \cdots+\frac{D_{1}}{2^{K-1}}+\frac{1}{2^K})V_{ref}$,
% \sum_{j=K-i+1}^{K-1} D_{j} 2^{j} +2^{K-i} -\frac{1}{2}
% $(2^{K-i}-\frac{1}{2})\text{LSB},  (D_{K-1}2^{K-1}+2^{K-2}-\frac{1}{2})\text{LSB} 
% \ldots, (D_{K-1}2^{K-1}+\cdots+D_{1}2^{1} + 1-\frac{1}{2})\text{LSB} $, 
\begin{equation}
        i = \begin{cases}
             (10,\ldots,0)_{2}, &k=1\\
             (\underbrace{ D_{K-1} \cdots D_{K-k+1}}_{k-1} 1 \cdots 0)_{2}, &otherwise
             \end{cases}
\end{equation}
successively, 
where $D_{i}$ is the $i$-th bit of the output code,
$(\cdot)_2$ is the binary representation of $i$th reference voltage at $k$-th step. 
For conventional Uniform (U) ADCs,
reference voltages are equally spaced ($(k-\frac{1}{2}) \cdot \text{LSB}, k=0,\ldots, 2^K-1$), 
and number of A/D operations is fixed.
In contrast, Non-uniform ADC (NU) performs BS on a customized grid,
which has a higher density in the range with more values
achieving lower bits and fewer A/D operations, as shown in Fig.~\ref{fig::sar_adc}~(b). 


\subsection{Motivation}
Previous work has tried to reduce the resolution of the ADCs 
by customizing non-uniform ADCs and parameters fine-tuning~\cite{sun2020energy}, %, ma2020tiny}. 
at the expense of the efforts in model training and ADC design.
% However, low bit-width results introduce a larger quantization error and greatly decrease the prediction accuracy. 
% Both re-training models and hardware customization require huge efforts. 
% Besides, to preserve the algorithm flexibility of the accelerator, 
% designers prefer 8-bit data bit-width, uniform quantization levels, and ADC with enough bit-width margin. 
Nowadays, more and more application cooperates with multiple deep neural networks to achieve state-of-the-art performance. 
Accelerators with overly customized ADCs are no longer competitive. 
For this reason, we do not want to modify the analog characteristics of ADC\@. 
% SAR ADC has the advantage of low power consumption and can easily achieve flexible resolution by changing the search logic. 
% As shown in Fig.~\ref{sar_adc}, SAR logic performs a binary search. 
% \begin{figure}[tbhp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{ims/pdf/sar_base.drawio.pdf}
%     \caption{Conventional SAR ADC}
%     \label{sar_adc}
%    % \Description{}
%     %\vspace{-0.4cm}
% \end{figure}
% In each \textbf{conversion step}
% \footnote[1]{To distinguish from the ``cycle'' of system clock, we use ``ADC cycle'' to represent the time of ``conversion step'' of ADC to generate one bit.\label{fn:adc}}, 
% the comparator compare DAC output ($V_{adc}$) and the sampled voltage ($v_{hold}$), and generate 1-bit result; 
% the binary result is fed to SAR logic sequentially to control DAC output in next \textbf{ADC cycle}~\footref{fn:adc}. 
% In this paper, we refer to the above process of generating 1-bit as one \textbf{A/D conversion}. 
% For a SAR ADC with $K$-bit resolution, it tasks K ADC cycles to generate maximum $K$-bit digital output. 

We are motivated to improve the ADC power consumption in a way that is orthogonal to the above techniques.
By profiling the distribution of the BL output values, 
we find a large proportion of redundancy bits in ADC output code from the perspective of numerical representation and characteristics of DNNs (Section~\ref{analysis}). 
There is a chance to compress the output code (Section~\ref{Methods}),
achieving adaptively resolution to reduce the ADC power consumption at the sub-conversion level. 
We find that the successive-approximation-register (SAR) ADC
can satisfy our aim. SAR ADC is one of the most mainstream ADC types in analog PIM macro, 
which features low circuit complexity and strongly benefits from process technology scaling. 
SAR ADC is more energy-efficient than other ADCs, such as flash ADC and pipeline ADC~\cite{murmann2012energy}. 
% SAR converters strongly benefit from small feature sizes (enabling small unit capacitances) and their relatively low circuit complexity (low digital and CV2-like overhead). 
% SAR ADC is a widely used ADC in analog PIM macro, due to the feature of low power consumption and high speed. 
The SAR ADC generates an N-bit binary code in N cycles by comparing the input voltage to a predefined sequence of voltage levels in a binary search. 
By modifying the logic part, SAR ADC can achieve flexible resolution. 
The output code compression can cooperate with SAR ADC by changing the searching logic (Section~\ref{hw-design}).


==> tex/3_analysis.tex <==
\section{Locate the redundant operations}\label{analysis}


\subsection{A/D operations and coding scheme}
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{ims/pdf/sar_base_2type.drawio.pdf}
    \caption{Conventional SAR ADC with (a) uniform and (b) non-uniform grid}%
    \label{fig::sar_adc}
\end{figure}
SAR logic performs a binary search 
to compare the input signal with a series of reference voltages generated by a digital-to-analog converter (DAC). 
Each comparison determines one bit of the output\footnote[1]{To distinguish from the ``cycle'' of the system clock, 
we use ``ADC cycle'' to refer to the time of ADC to generate one bit.\label{fn:adc}}, 
starting from the most significant bit (MSB) to the least significant bit (LSB).
The closest output level is used as the approximation of the sampled voltage.
$N$ bits are generated in $N$ ADC cycles, 
and \textit{the output code is the concatenation of the results of each search step}\footnote[2]{We refer to each step of generating 1-bit as one \textbf{A/D operation}, 
and the full progress as the \textbf{A/D conversion}}.

As shown in Fig.~\ref{fig::sar_adc}, the horizontal dash grid represents the output levels of DAC\@, 
the arrows represent searching traces, the points represent the sampled values to be sensed out, 
and the vertical dash grid represents the time steps. 
Conventional SAR ADCs perform a Binary Search (BS) on a Uniform (U) grid, as shown in Fig.~\ref{fig::sar_adc}~(a). 
Similarly, non-uniform ADC performs BS on a Non-Uniform (NU) grid that has higher density in the range with more values, 
achieving lower bits and fewer A/D operations, as shown in Fig.~\ref{fig::sar_adc}~(b).

\subsection{Value distribution at BLs and redundancy}
% It is usually considered that the activation values in neural networks are Gaussian distributed~\cite{Low_bit_quant_iccvw2019}. 
% However, the output of the ReRAM crossbar's BLs has yet to be systematically analyzed. 
% The distribution of the BLs is demonstrated in Fig.~\ref{non_uniform}, %Figure~\ref{distribution}, 
% which shows a very unbalanced distribution where most of them are very close to zero. 
% From an information-theoretic perspective, it is inefficient to encode non-uniformly distributed data with a fixed-length encoding scheme. 
% From a statistical perspective, by sacrificing the accuracy of the values in the minority, 
% it is possible to achieve fewer bits with only small errors on the whole. 
%
% While it is generally assumed that the activation in neural networks follows a Gaussian distribution~\cite{Low_bit_quant_iccvw2019}, 
% the output of the ReRAM crossbar's BLs has not been thoroughly examined. 
% Fig.~\ref{non_uniform} demonstrates the distribution of the BLs, 
% revealing a highly imbalanced distribution in which most samples are very close to zero. 
% From an information-theoretic standpoint, encoding non-uniformly distributed data using a fixed-length encoding scheme is inefficient.
% Also, sacrificing the accuracy of values in the minority can lead to fewer bits with only small errors overall, 
% as viewed from a statistical perspective.
% Consequently, we define the \textbf{redundancy} from two aspects: 
% \begin{itemize}
%     \item Neural networks are intrinsically fault-tolerant due to their nature redundancy\cite{torres2017fault}. 
%     From this aspect, some A/D conversion is redundant because they are not necessarily too accurate (\textbf{precision redundancy}). 
%     \item Also, the output values with higher frequency can be represented with less bit, i.e., cost fewer A/D operations (\textbf{representation redundancy}). 
% \end{itemize}

% Non-uniform quantization seems a good choice. 
% % \az{Defects of non-uniform quantization steps, from Hardware and software perspective}
% However, the unconstrained non-uniform quantization and the optimal prefix code, like Huffman code, 
% are not easy to be processed by hardware because the codebooks are required for decoding. 
% Huffman coding is a particular type of optimal prefix code that is commonly used for lossless data compression. 
% Input values are separated into component symbols, and each is replaced with a variable-length code; more common symbols are represented with fewer bits than less common symbols. 
% \uline{This enlightens us to reduce redundant A/D operations by using the output coding scheme with higher efficiency for ADC\@. } 
% \begin{figure}[tbhp]
%     \centering 
%     \includegraphics[width=0.8\linewidth]{ims/pdf/searching_strategy_w_stat.pdf} 
%     \caption{Various searching strategies. (a) binary search with uniform grid, (b) binary search with non-uniform grid, (c) biased search, 
%     (d) search with early stopping, (e) search with pre-detection}%
%     \label{fig::searching}
%    % \Description{}
% %    \vspace{-0.5cm} 
% \end{figure} 
% We find \textbf{two opportunities} to \uline{achieve 
% both lower coding length and flexible sensing resolution can be achieved, 
% by changing the searching strategy} of an ``over-accurate ADC'', 
% which has a higher resolution than is required. 
% \begin{enumerate}
%     \item 
%     For values with high frequency and are concentrated in a small interval, we call them ``early birds''.     
%     Because a small interval contains fewer candidates, the closest level of the samples can be found in fewer steps. 
%     If we pre-detect ``early birds'' with an additional phase (Fig.~\ref{fig::searching} (a)) 
%     or compare the samples with candidates in the target interval in a higher priority (Fig.~\ref{fig::searching} (c)), 
%     bits (of A/D operations) needed by ``early birds'' is reduced with no precision loss. 
%     % \item Similarly, reduced sensing precision can also be achieved by early stopping the conversion progress, as shown in Fig.~\ref{fig::searching} (d). 
%     % This strategy provides the opportunity to explore the redundant bits that are not needed by fault-tolerant neural networks. 
%     \item 
%     Fig.~\ref{fig::searching} (b) illustrates how early stopping of the conversion progress can achieve reduced sensing precision. 
%     This strategy presents an opportunity to explore redundant bits that are unnecessary for overall accuracy.
% \end{enumerate}
% Based on the observation above, to improve the energy efficiency of the ReRAM analog computing, 
% we aim to find a configurable quantization scheme that is suitable for ADC design and can reduce the redundant A/D conversion efficiently. 

While it is commonly assumed that the activation in neural networks follows a Gaussian distribution~\cite{Low_bit_quant_iccvw2019}, 
the output of the ReRAM crossbar's BLs has not been thoroughly investigated. 
Fig.~\ref{non_uniform} illustrates the distribution of the BLs, 
revealing a highly imbalanced distribution where the majority of samples are very close to zero. 
From an information-theoretic perspective, encoding non-uniformly distributed data using a fixed-length encoding scheme is inefficient. 
Additionally, sacrificing the accuracy of values in the minority can result in fewer bits with only small errors overall, 
as observed statistically.
Hence, we define \textbf{redundancy} from two aspects:
\begin{itemize}
\item Neural networks inherently possess fault tolerance due to their redundant nature~\cite{torres2017fault}. 
Consequently, some A/D operations are redundant since they do not require excessive accuracy (\textbf{precision redundancy}).
\item Moreover, values with higher frequencies in the output can be represented with fewer bits, 
thereby reducing the number of required A/D operations (\textbf{representation redundancy}).
\end{itemize}

Non-uniform quantization is a favorable option. However, unconstrained non-uniform quantization and optimal prefix codes, such as Huffman codes, 
pose challenges in hardware processing due to the need for codebooks for decoding. 
Huffman coding is a specific type of optimal prefix code commonly used for lossless data compression. 
It divides input values into component symbols, 
replacing each symbol with a variable-length code, 
where more common symbols are represented with fewer bits compared to less common symbols. 
This insight leads us to reduce redundant A/D operations 
i.e., $N_{A/D\_ops}$ in $E_{convert} = e_{\text{op}} N_{A/D\_ops}$,
($e_{\text{op}}$, and $N_{A/D\_ops, i}$ represent energy per A/D operation, 
and the number of A/D operations required by each conversion, respectively),
by utilizing an output coding scheme that offers higher efficiency for ADC\@.
\begin{figure}[tbhp]
    \centering 
    \includegraphics[width=0.7\linewidth]{ims/pdf/searching_strategy_new.drawio.pdf} 
    \caption{Heuristic searching strategies overcoming redundancy. (a) biased search, (b) search with early stopping}%
    \label{fig::searching}
   % \Description{}
%    \vspace{-0.5cm} 
\end{figure} 
We have identified two opportunities to achieve both shorter coding length and flexible sensing resolution by changing the searching strategy of an ``over-accurate ADC'', which has a higher resolution than necessary:
\begin{itemize}
    \item 
    By profiling we can identify a small interval that contains the majority of the samples.
    If a sample can be pre-detected in such an interval, 
    the closest level of the samples can be found in relatively fewer steps\footnote[3]{Even though an extra detection phase is introduced},
    We refer to these samples as ``early birds'', as shown in Fig.~\ref{fig::searching}(a).
    The A/D operations required by ``early birds'' can be reduced with no precision loss.
    \item ``Early stopping'', in contrast,
        stops the conversion progress even though the output code is not fully determined, 
        resulting in reduced sensing precision, as shown in Fig.~\ref{fig::searching}(b).
        This strategy enables the exploration of redundant bits that are unnecessary for overall accuracy.
\end{itemize}

Based on these observations, our goal is to find a configurable quantization scheme that is suitable for ADC design and efficiently reduces redundant A/D operations to enhance the energy efficiency of ReRAM analog computing.

==> tex/5.5_related.tex <==
\section{Related works} 
% We compare our work with two SOTA works (1). He, Yintao, et al. InfoX. DAC22 (2) Li, Xingchen, et al. Tailor DAC22. 
{InfoX}~\cite{He22Infox} defines this redundancy from the perspective of numerical representation.
It truncates the output outlier value ($\mu \pm 3\sigma$) and finds the maximum bit-width can retain 80\% Information entropy.
{Tailor}~\cite{Li22Tailor} defines the redundant bits as those that do not contribute to the next level input.
Ours, instead, from the perspective of quantization methodology, defines redundancy as the ADC operations contributing less to overall accuracy. 
The proposed quantization method perfect perfectly compatible with the SAR-ADC design.
Similarly, we are all motivated to reduce the ADC energy consumption in ReRAM-based DNN accelerators. ADC converts analog MVM to digital values.
The numerical-lossless precision is redundant. 
{RAELLA}~\cite{Andrulis2023RAELLA} modifies the arithmetic and slicing operations in the crossbars to produce low-resolution analog results that can be converted by low-resolution ADCs with minimal loss of accuracy. 
In {ISAAC}~\cite{shafiee2016isaac}, weight encoding is employed, where large weights are ``flipped'' by subtracting them from $2^N -1$ to obtain smaller conductance values.

Although we are all focusing on enabling efficient PIM inference without retraining, 
our method also preserves the flexibility of the hardware, 
squeezing the bit-level redundancy during each convention. 
Further, our quantization method is orthogonal to all of these works,
the conversion function is configured by the digital logic in the ADC\@.


==> tex/7_apped.tex <==
\appendix 
Solve a 2D bin-packing problem with Google OR tools: 
N items of various shapes need to be packed into M bins with the same width but various heights. 
Inputs:
1. Bin set, $\mathcal{B}$, in which each bin has shape $W_max, H_max_j, j \in 1, \ldots M$, 
2. Rectangle set, $\mathcal{R}$, in which each item has shape $w_i,h_i, i \in 1, \lodts, N$.

% Variables:
% \beign{enumerate}
%     \item $a_i,b_i$, the coordinates of the lower-left corner of each item. 
%     \item $x[i][j]$ whose value is 1 if the item i is placed in bin j, and 0 otherwise.
%     \item $y[j]$, whose value is 1 if bin j is used—that is if any items are packed in it—and 0 otherwise. 
%     \item big-M relaxation and auxiliary variables $z^k_{i,j} \in {0, 1}, k = 1, \lodts , 4$
% \end{enumerate}

% Constraints: 
% 1. To make sure that no two overlap, for any two items $B_i, B_j \in \mathcal{B}, i < j$, ensure that
% $(a_i + w_i \leq a_j ) \lor (a_j + w_j \leq a_i) \lor (b_i + h_i \leq b_j ) \lor (b_j + h_j \leq b_i)$.
% 2. Ensure the rectangle containment: for any item i that is placed in bin j, any dimension cannot exceed the bin size in both width and height, 
% $(a_i + w_i \leq W\_max ) \land (b_i + h_i \leq H\_max_{j} ) $
% 3. Each item must be in exactly one bin, $\sum_{i=1}^{N} x[i][j]=1$
% Target: 
% minimize the total height, i.e., $\sum_{j=1}^{M} y_j * H\_max_{j}$ .

